Against the Others! Detecting Moral Outrage inSocial Media Networks

Online firestorms on Twitter are seemingly arbitrarily occurring outrages towards people, companies, media campaigns and politicians. Moral outrages can create an excessive collective aggressiveness against one single argument, one single word, or one action of a person resulting in hateful speech. With a collective "against the others" the negative dynamics often start. Using data from Twitter, we explored the starting points of several firestorm outbreaks. As a social media platform with hundreds of millions of users interacting in real-time on topics and events all over the world, Twitter serves as a social sensor for online discussions and is known for quick and often emotional disputes. The main question we pose in this article, is whether we can detect the outbreak of a firestorm. Given 21 online firestorms on Twitter, the key questions regarding the anomaly detection are: 1) How can we detect the changing point? 2) How can we distinguish the features that cause a moral outrage? In this paper we examine these challenges developing a method to detect the point of change systematically spotting on linguistic cues of tweets. We are able to detect outbreaks of firestorms early and precisely only by applying linguistic cues. The results of our work can help detect negative dynamics and may have the potential for individuals, companies, and governments to mitigate hate in social media networks.

==> junk.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% taken out of introduction, rel work and analysis.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

19/4/20
We argue that from a social scientist point of view sudden bursts of communication are interesting to focus on with regards of collective crowd behavior. 
The analyses of our article use these online firestorms as starting point to follow up on their research findings in order to advance knowledge about firestorms and the spread of rumors. We build up on this research by tackling the problem of life time monitoring features of anomaly in the network.
In order to address our research question of detecting the starting event as a change point of an outrage, we use extracted characteristics of the mention network.

disc
Our research question was about detecting anomaly in a network and exploring the major features that indicate the outbreak of a firestorm, hence starting point of possible collective action.
We found out that that the maximum in-degree in mention networks means the highest number of mentions received by a particular user. Thus,  the  ability  of  this  feature  to  detect  a  firestorm  can  be interpreted by considering that, generally speaking, a firestorm occurs when one user is being mentioned unusually high
We further evaluated the change-point-detection systematically measuring the interval between the outbreak of the firestorm and the begin/end of the corresponding period between two change points. We looked for a change point con-figuration with which the peak of the firestorms lies between two change points.
This suggests that, the frequency of  @mentions over time in hashtags and retweets are valuable indicators of anomaly. Regarding this point of change where a sudden burst emerges 
Valuable results for collective action?

conclusion
To answer our aforementioned research questions we can state that we can detect a changing point focusing on the evolution of time. We propose a novel change detection model that spots on time series analysis in the mention network for all given firestorms.
To provide rich information on an outbreak of a moral outrage in online discussions, we use extracted characteristics from the mention network to detect the outbreak at an early stage. With our method we can detect firestorms in real time Twitter data by only monitoring ...

18/4/20
Assuming that a firestorm affects user positively or negatively, we might see changes in their use of language, more precisely in their textual comments as tweets in the mention network. It is generally accepted that in  speaking we perform actions of various kinds and so we might see changes in the way people speak. While speech acts as performative acts contain verbs that indicate the action, pronouns indicate to whom the action is performed. In this way we might figure out to whom and how the outrage starts. 

In order to address our research question of the relationship between speech acts and firestorm participation, we use the extracted characteristics of firestorms to detect an outbreak at an early stage. Our approach provides a method from network analysis and text statistics by examining the dynamics of linguistical cues over time. We evaluate the sentiment score for each tweet in comparison to the overall network and evaluate the pronouns of each tweet of an user as an indicator for changing speech acts. We analyzed tweets from the week before the firestorm and the week during the firestorm.

We use the LIWC2015 processing Tool to extract the positive and negative values of tweets and the usage of the LIWC categories such as personal pronouns, affective processes, cognitive processes and perceptual processes and informal language. We combine positivity and negativity metrics with linguistical cues to the network effects. Lexical features have been widely explored in the psychological and computational literature. For these features we drew mainly on the LIWC lexicons of Pennebaker et al. (2015), the standard for social psychological analysis of lexical features. 

In our method we do not limit our analysis to just sentiments and emotional tone since it is questionable to examine the correct meaning of a tweet out of counting words. Comparing the firestorm data manually to the LIWC analysis, we found out that many cynical statements were not captured as such. Relying simply on this valence would not give much insights about the emotional arousal of a users textual comment. 
On this account, we assume that detecting change on sentiment plus the usage of pronouns is more significant in how people connect with each other to form an outrage. The usage of pronouns gives insights about how a user connects himself with others. Function words are psychologically and linguistically interesting and have been studied broadly. \cite{Benveniste1966} gives theoretical background on the nature of pronouns. They are used at high rates. Function words require social skills to use properly. The speaker assumes the listener knows who everyone is and the listener must know the speaker to follow the conversation. The ability to understand a simple conversation packed full of function words demands social knowledge. All function words work in this way. The ability to use them is a marker of basic social skills – and analysing how people use function words reveals a great deal about their social worlds. \cite{Pennebaker2011}

Refs:
Sentiment analysis was applied by \cite{Brady2017} to analyze the emotional shape of moral discussions in social networks. They argue that moral-emotional language increased diffusion more strongly. Highlighting the importance of emotion in the social transmission of moral ideas, they demonstrate the utility of social network methods for studying morality.\cite{Ferrara2015} instead, measures emotional contagion in social media and networks by evaluating the emotional valence of content the users are exposed to before posting their own tweets. \cite{Charlton2016} developed a model of collective sentiment on Twitter. 
A different approach was used by \cite{Bail2017} who use sentiment analysis measuring the frequency of cognitive and emotional language on Facebook and argue that rational and emotional styles of communication have strong influence on conversational dynamics. Linguistic pattern analysis was used by \cite{Sharp2004} to analyze affective arousal and linguistic output. Patterns of word choice were used by \cite{Shaikh2017} in an online social platform reflecting on pronouns to characterize how a community forms in response to adverse events such as a terrorist attack. In a study of\cite{Gonzales2010} the authors found out that synchronized verbal behavior can reveal important information about social dynamics. The study demonstrates the effectiveness of using language to predict change in social psychological factors of interest.

Conclusion
overall emotionality and the linguistic cues such as the usage of pronouns.
With the linguistic features that contains network information we were able to see how mention networks evolve over the two weeks.

Further questions
Can we see unifying processes within the user interaction beyond the firestorm?

The dependent variable is the changing (or evolving) relation network, represented by two or more observations of a directed graph with a fixed set of actors. The network evolution is modeled as the consequence of the actors making new choices, or withdrawing existing choices, on the basis of functions, with fixed and random components, that the actors try to maximize.


With the analysis using LIWC, we got many new attributes of tweets, including positive and negative emotions. The following figure shows the evolution of those attributes (average per tweet) over time. Evolution of positive and negative emotions over time
\includegraphics[width=.4\textwidth]{emotion_evolution.pdf}
We have also constructed mention networks and retweet networks. For each type we have two versions:
\begin{itemize}
\item independent: where a network at each hour is constructed independently
\item accumulative: where for each hour, all the mentions from the beginning of the event are used.
\end{itemize}
This figure shows how the accumulative mention networks evolve over time (in terms of nodes N and edges)
\includegraphics[width=.4\textwidth]{ment_net_NE.pdf}

This one shows the evolution of number of weakly connected components (nwcc), and strongly connected components (nscc) (where SCC of size 1 were omitted) over time, for accumulative mention networks.
\includegraphics[width=.4\textwidth]{ment_net_ccs.pdf}

This one shows how k-cores of accumulative mention networks develop over time, in terms of size and k:
%ment_net_kcore.pdf

In order to get more insight on how the discussions (via mentions) go throughout the event, we extracted, for each event, a sub-network contains reciprocated mentions only (regardless of time). The results of analyzing those sub-networks are the following:
Table \ref{tab:sub-recp-ment} shows the attributes of reciprocated mentions networks: number of nodes (N), edges (E), connected components (CC), and the size of the largest connected components (LCC), and the number of messages (msgs) that make up the network. Those networks are:
1. very small in size relative to the entire event (users, tweets, and mentions)
2. consists mainly of few, small connected components, which means:  short conversions among small number of users (2-3).

One exception is the event `suey park'. This means that the events at hand, although huge in number of messages, are not actually real conversations/discussions.

\begin{table}[]
\centering
\caption{Characteristics of sub-networks with reciprocated mentions}
\label{tab:sub-recp-ment}
\begin{tabular}{l| r r | r r | r}
      & N & E & CC & LCC & msgs \\
\hline 
askbg     & 8 & 4 & 4 & 2 & 8 \\
askjpm    & 17 & 9 & 8 & 3 & 21 \\
askthicke & 10 & 5 & 5 & 2 & 10 \\
cancelcolbert & 58 & 39 & 19 & 21 & 114 \\
celebboutique & 40 & 20 & 20 & 2 & 41 \\
david\_cameron & 46 & 23 & 23 & 2 & 58 \\
fafsa       & 21  & 12 & 9 & 5 & 30 \\
gaelgarciab & 22  & 12 & 10 & 3 & 31 \\
klm         & 116 & 70 & 50 & 7 & 175 \\
mcdstories  & 2   & 1 & 1 & 2 & 2 \\
muslimrage  & 52  & 27 & 25 & 3 & 61 \\
mynypd      & 45  & 24 & 21 & 3 & 55 \\
notintendedtobeafactualstatement & 18 & 9 & 9 & 2 & 21 \\
qantas       & 60 & 35 & 25 & 5 & 91 \\
qantasluxury & 13 & 7  & 6  & 3 & 15 \\
spaghettios  & 35 & 18 & 17 & 3 & 43 \\
suey\_park      & 361 & 361 & 62 & 206 & 1768 \\
theonion        & 106 & 56 & 51 & 3 & 140 \\
ukinusa         & 2  & 1 & 1 & 2 & 2 \\
voguearticles   & 0  & 0 & 0 & N/A & 0  \\
whyimvotingukip & 49 & 25 & 24 & 3 & 53 \\
\end{tabular}
\end{table}


\begin{figure*}[]
\centering
\includegraphics[width=\textwidth]{images/emotion_evolution_2.pdf}
\caption{Emotionality (pos and neg) evolution DURING firestorms (moving average over a window of 5 hours)}
\label{fig:my_label}
\end{figure*}


%Mirco
Regarding networks we correlated adjacency matrices with matrices of sentiments. We have correlated the adjacency information and emotionality of connections.

\includegraphics[width=.4\textwidth]{correlating_matrices.pdf}

The dots represent two correlation coefficients for the time before (x-axis) and during (y-axis) the firestorms.
Emotionality means positive emotion + negative emotion. For other evaluations, we decided to subtract negemo from posemo.
We also ignored all zero entries in the adjacency matrix meaning we only considered existing edges when extracting the sentiments.
One can see that before the firestorms, there were slight correlating effects in the number of mentions and emotionality. these effects vanish during the firestorms - here, most of the correlation coefficients drop below $0.25$. One remarkable exception is again the suey park storm.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\if F
Figure \ref{fig:chgpnt_until_detection} visualizes nicely the predicted change point, the one that is closest to the peak of the firestorm when the firestorm is already taking place. For suey-park, for example, we detect a change point around 15 hours before the peak. At that point, \#suey-park was already among the top 10 hashtags.
Up to askbg, we're well below 5 hours away from the peak, which is in 16 out of 20 cases.

\begin{figure}[t]
\includegraphics[width=.9\linewidth]{images/stream_t_detection_of_fs.pdf}
\centering
\caption{relevant changepoints closest to peak}
\label{fig:chgpnt_until_detection}
\end{figure}
\fi

==> sections/analysis_junk.tex <==

To evaluate the change-point-detection systematically, we measured the interval between the outbreak of the firestorm and the begin/end of the corresponding period between two change points. Since the change point detection can be quite noisy, it is challenging to define the period of a firestorm automatically. 

Instead, we looked for a change point configuration with which the peak of the firestorms lies between two change points (Fig. 5?). The result can be seen in the firestorm muslimrage (Fig. 7) %(new visualization with smoothed signal). 
In Fig. 6 a bar of a period of a mean covers a big part of the firestorm. For other firestorms and other sentiments like 'i' and 'we', this often yields good results. We looked at some of them manually.
% But now I'm wondering how to evaluate that systematically. When is this a good result? 
Measuring the time between the peak of the firestorm and the change point at the beginning of the highlighted bar, the distribution of intervals can be found in the other plot. %which one?
We are often very close to the peak. 
%Or should we label the beginning and the end of the firestorm manually for evaluation purposes?

%\includegraphics[width=.4\textwidth]{changepoint_to_outbreak.pdf}

%This belongs to Fig. 7?



Focusing on the intervals between change points and peaks of firestorms in the evaluation (Fig. 6), we can argue that a combination of predictors yields good results, i.e. observing the overall emotionality together with the usage of 'i'. Observing negative emotion does not give valuable results. Attached is another example where the outbreak was captured quite clearly. %is there a figure?

%Should we have some form of combined evaluation where we put together all our predictors and see how a combination performs? Or would this be alright?

%\includegraphics[width=.4\textwidth]{chdtct_gaelgarciab_i.pdf}
%\includegraphics[width=.4\textwidth]{chdtct_mcdstories_emo.pdf}
%\includegraphics[width=.4\textwidth]{chdtct_gaelgarciab_negemo.pdf}

==> sections/discussion.tex <==
Our research question tackled the detection of anomaly in a network and exploring the major features that indicate the outbreak of a firestorm, hence, the starting point of possible collective changing behavior.
We found out that that the maximum in-degree in mention networks means the highest number of mentions received by a particular user. Generally speaking, a firestorm occurs when one user is being mentioned unusually high.
Based on lexical features, we further evaluated the change-point-detection systematically measuring the interval between the outbreak of the firestorm and the begin/end of the corresponding period between two change points. We are able to detect a change in the linguistic behavior of the users very closely. ja,
Before the outbreak of the firestorms, the users mention an 'I' noticeably often with positive emotion, whereas during the firestorms the mentioning of 'I' completely vanishes together with a rise of negativity. 
The use of words change at a certain point when users stop commenting with the I-perspective. As mentioned, pronouns refer to a referent. If the 'I' diminishes, the focus changes significantly. All of a sudden people stop talking collectively about themselves and collectively - against the others. That came up clearly with our analysis. Now, our model picks up these features and is able to detect the starting point of outrages giving insights about the changing user perspective from "one against the others".
